Solving Partial Differential Equations Using Artificial Neural Networks

Partial differential equations have a wide range of applications in modeling multiple physical, biological, or social phenomena. Therefore, we need to approximate the solutions of these equations in computationally feasible terms. Nowadays, among the most popular numerical methods for solving partial differential equations in engineering, we encounter the finite difference and finite element methods. An alternative numerical method that has recently gained popularity for numerically solving partial differential equations is the use of artificial neural networks. Artificial neural networks, or neural networks for short, are mathematical structures with universal approximation properties. In addition, thanks to the extraordinary computational development of the last decade, neural networks have become accessible and powerful numerical methods for engineers and researchers. For example, imaging and language processing are applications of neural networks today that show sublime performance inconceivable years ago. This dissertation contributes to the numerical solution of partial differential equations using neural networks with the following two-fold objective: investigate the behavior of neural networks as approximators of solutions of partial differential equations and propose neural-network-based methods for frameworks that are hardly addressable via traditional numerical methods. As novel neural-network-based proposals, we first present a method inspired by the finite element method when applying mesh refinements to solve parametric problems. Secondly, we propose a general residual minimization scheme based on a generalized version of the Ritz method. Finally, we develop a memory-based strategy to overcome a usual numerical integration limitation when using neural networks to solve partial differential equations.

==> Chapters/0.Chapter/basque_title.tex <==
% !TEX root = ../../main.tex

%Basque title
\begin{titlepage}
\vfill
\begin{center}
\includegraphics[height=2.5cm]{logo_bcam.png}
\hfill
\includegraphics[height=2.5cm]{logo_upv.jpg}\\
\vspace{2cm}
\textit{Doktorego tesia}\\
\vspace{1cm}
{\Huge {\textsc{{\begin{minipage}{\textwidth}\hrulefill\begin{center}\vspace{0.3cm}\titleEU\end{center} \hrulefill \end{minipage}}}}}
\end{center}
\begin{center}
\vspace{2cm}
{\Huge{\textsc{\author}}}\\
\vspace{2cm}
{\large\textsc{Zuzendariak: \supervisors}\\
\vspace{2cm}
2023}
\end{center}
\end{titlepage}









==> Chapters/0.Chapter/instructions.tex <==
% !TEX root = ../../main.tex

%\mbox{}
%\begin{titlepage}
\vspace*{\fill}

\selectlanguage{english}
This dissertation is written in English and Basque. In the part prior to the main body, the mixture of languages obeys the following rule: for contents with a single paragraph, two paragraphs will appear---the first one in English and the second one in Basque. For contents with more than one paragraph, they will be distinguished by subsections entitled in either English or Basque. In the body of the dissertation, odd chapters are developed in Basque while even chapters are in English. To internationalize the scope of the presented work, the appendices include the English translations of the odd chapters written in Basque.

\selectlanguage{basque}
Tesi hau ingelesez eta euskaraz idatzita dago. Tesiaren gorputzaren aurreko zatian, hizkuntzen nahasketak honako arau hau beteko du: bi paragrafo agertuko dira (lehenengoa ingelesez eta bigarrena euskaraz) testu-paragrafo bakarra duten edukietan. Paragrafo bat baino gehiagoko edukiak aldiz, ingelesezko edo euskarazko izenburua duten azpiatalen bidez bereiziko dira. Tesiaren gorputzean, kapitulu bakoitiak euskaraz garatuko dira, eta kapitulu bikoitiak, ingelesez. Aurkeztutako lanaren irismena nazioartera zabaltzeko xedez, euskarazko kapitulu bakoitien ingelesezko itzulpenak eranskinetan jasoko dira.
%\end{titlepage}

==> Chapters/0.Chapter/main_title.tex <==
% !TEX root = ../../main.tex

\newcommand{\titleEN}{Solving Partial Differential Equations using Artificial Neural Networks}
\newcommand{\titleEU}{Deribatu partzialetako ekuazioen ebazpena neurona-sare artifizialen bidez}
\renewcommand{\date}{2023}
\renewcommand{\author}{Carlos Uriarte}
\newcommand{\supervisors}{David Pardo, Elisabete Alberdi}

%Main title
\begin{titlepage}
\vfill
\begin{center}
\begin{center}
\includegraphics[height=3cm]{logo_upv.jpg}
\end{center}\vspace{1cm}
\begin{minipage}[t]{0.49\textwidth}
\centering
\textit{Ph.D. Dissertation}
\end{minipage}\hfill
\begin{minipage}[t]{0.49\textwidth}
\centering
\textit{Doktorego tesia}
\end{minipage}
\vspace{0.5cm}
\end{center}
\begin{center}
{\Huge {\textsc{\begin{minipage}{\textwidth}\hrulefill \begin{center}\vspace{0.3cm}\titleEN\begin{center}\rule{0.5\textwidth}{.4pt}\vspace{0.3cm}\end{center}\titleEU\end{center}\hrulefill\end{minipage}}}}
\end{center}
\begin{center}
\vspace{1.5cm}
{\LARGE{\textsc{\author}}}\\
\vspace{1.5cm}
\date
\end{center}
\end{titlepage}







==> Chapters/2.Chapter/analytic_case_english.tex <==
\newpage
\section{An analytic case of study using FFNNs}\label[appendix]{appendix2}

We follow the notation and terminology introduced in \Cref{section1.3} along the entire study.

At the continuum level,  let $X:=(-1,1)$,  $Y:=\mathbb{R}$,  and
\begin{equation}
u^*(x):=\text{sgn}(x)=\begin{cases}-1,&\text{if } x<0,\\ \phantom{-}0,&\text{if } x=0,\\ \phantom{-}1,&\text{if } x>0.\end{cases}
\end{equation} Consider $\mathbb{U}:=L^2(X)=\{u:X\longrightarrow \mathbb{R} : \int_X u^2 <\infty\}$ and let 
\begin{equation}\label{Chapter1_case_study}
\mathcal{F}(u):=\Vert u-u^*\Vert_{L^2(X)}^2=\int_X (u(x)-u^*(x))^2 \ dx,
\end{equation} whose minimum in $\mathbb{U}$ is zero and is attained only at $u^*$.

At the parameterization level,  let $\Theta:=\mathbb{R}^2$ and let $u_\text{NN}:X\times\Theta\longrightarrow\mathbb{R}$ be defined by
\begin{equation}
u_\text{NN}(x;\theta):=c\tanh(ax),
\end{equation} where $\theta=\{a,c\}$ denotes the set of learnable parameters.  Then,  
\begin{equation}
\mathbb{U}_\text{NN}=\Phi_\text{NN}(\Theta)=\{\Phi_\text{NN}(a,c) = c\tanh(ax):X\longrightarrow Y\}_{a,c\in\mathbb{R}}, 
\end{equation} and routinary calculations yield
\begin{align}
(\mathcal{F}\circ\Phi_\text{NN})(a,c)&= 2(1+c^2) - \frac{4c\log(\cosh(a))+2c^2\tanh(a)}{a},  \label{Chapter1_objetive_function}\\
\frac{\partial(\mathcal{F}\circ\Phi_\text{NN})}{\partial a}(a,c)&= \frac{2c\left( 2\log(\cosh(a))+ (c-2a)\tanh(a)- ac(\text{sech}^2(a)\right)}{a^2}, \\
\frac{\partial(\mathcal{F}\circ\Phi_\text{NN})}{\partial c}(a,c)&= \frac{4\left(ac-\log(\cosh(a))-c\tanh(a)\right)}{a},
\end{align} for $a\neq 0$,  $(\mathcal{F}\circ\Phi_\text{NN})(0,c)=2$,  $\frac{\partial(\mathcal{F}\circ\Phi_\text{NN})}{\partial c}(0,c)=-2c$,  and $\frac{\partial(\mathcal{F}\circ\Phi_\text{NN})}{\partial a}(0,c)=0$.  \Cref{Chapter1_analytic_F} shows the graph of $\mathcal{F}\circ\Phi_\text{NN}$,  and \Cref{Chapter1_analytic_gradF} shows the graphs of its partial derivatives.  

\begin{figure}[htbp]
\centering
\begin{subfigure}{\textwidth}
\centering
\begin{tikzpicture}
\begin{axis}[width=0.7*\textwidth,  view = {35}{55},  colorbar,  colorbar style={fill opacity=0.4, tick label style={opacity=1}}, xlabel = {$a$}, ylabel={$c$}, ytick={-4,-2,0,2,4},zlabel={$(\mathcal{F}\circ\Phi_\text{NN})(a,c)$},ztick={0,25,50}]
 \addplot3[surf, opacity=0.4, domain=-5:5,  samples=50,
 ]{2*(1+y^2)-(4*y*ln(cosh(x))+2*y^2*tanh(x))/x};
\end{axis}
\end{tikzpicture}
\end{subfigure}
\vskip 1em
\begin{subfigure}{\textwidth}
\centering
\begin{tikzpicture} 
\begin{axis}[width=0.7*\textwidth,  view = {0}{90},  colorbar,  colorbar style={fill opacity=0.5, tick label style={opacity=1}}, xlabel = {$a$}, ylabel={$c$}, title={$(\mathcal{F}\circ\Phi_\text{NN})(a,c)$}]
    \addplot3 [surf, shader = interp, opacity=0.4, domain=-5:5, samples=50,
 ]{2*(1+y^2)-(4*y*ln(cosh(x))+2*y^2*tanh(x))/x};
\end{axis}
\end{tikzpicture}
\end{subfigure}
\caption{Graph of $\mathcal{F}\circ \Phi_\text{NN}$ for \eqref{Chapter1_case_study} from two different perspectives.}
\label{Chapter1_analytic_F}
\end{figure}

\begin{figure}[htbp]
\centering
\begin{subfigure}{\textwidth}
\centering
\begin{tikzpicture} 
\begin{axis}[width=0.7*\textwidth,  view = {0}{90},  colorbar,  colorbar style={fill opacity=0.5, tick label style={opacity=1}}, xlabel = {$a$}, ylabel={$c$}, title={$\displaystyle \frac{\partial(\mathcal{F}\circ\Phi_\text{NN})}{\partial a}(a,c)$}]
    \addplot3 [surf, shader = interp, opacity=0.4, domain=-5:5, samples=50,
 ]{(2*y/x^2)*(2*ln(cosh(x))+ (y-2*x)*tanh(x)- x*y*(1-(tanh(x))^2))};
     \draw[color=black, line width=0.8, dashed] plot[variable=\x,  domain=-5:5,samples=5,smooth] (\x,  0,1);
     \draw[color=black, line width=0.8, dashed] plot[variable=\x,  domain=-5:-0.1,samples=50,smooth] (\x,  {2*( ln(cosh(\x)) - \x * tanh(\x) ) / ( \x * ( 1 - (tanh(\x))^2 ) - tanh(\x) )},  1);
     \draw[color=black, line width=0.8, dashed] plot[variable=\x,  domain=0.1:5,samples=50,smooth] (\x,  {2*( ln(cosh(\x)) - \x * tanh(\x) ) / ( \x * ( 1 - (tanh(\x))^2 ) - tanh(\x) )},  1);
     \node (a) at (1.9,-1.3) {$c=\frac{2(\log(\cosh(a)) - a\tanh(a))}{a \text{ sech}^2(a) - \tanh(a))}$};
     \node (b) at (-2,0.5) {$c=0$};
     \draw[->] (a) -- (3, {2*( ln(cosh(3)) - 3 * tanh(3) ) / ( 3 * ( 1 - (tanh(3))^2 ) - tanh(3) )-0.2});
     \draw[->] (a) -- (-0.25,{2*( ln(cosh(-0.4)) - (-0.4) * tanh(-0.4) ) / ( -0.4 * ( 1 - (tanh(-0.4))^2 ) - tanh(-0.4) )}); 
\end{axis}
\end{tikzpicture}
\end{subfigure}
\vskip 1em
\begin{subfigure}{\textwidth}
\centering
\begin{tikzpicture} 
\begin{axis}[width=0.7*\textwidth,  view = {0}{90},  colorbar,  colorbar style={fill opacity=0.5, tick label style={opacity=1}}, xlabel = {$a$}, ylabel={$c$}, title={$\displaystyle \frac{\partial(\mathcal{F}\circ\Phi_\text{NN})}{\partial c}(a,c)$}]
    \addplot3 [surf, shader = interp, opacity=0.4, domain=-5:5, samples=50]{(4/x)*(x*y-ln(cosh(x))-y*tanh(x))};
     \draw[color=black, line width=0.8, dashed] plot[variable=\x,  domain=-5:5,samples=5,smooth] (0, \x,1);
     \draw[color=black, line width=0.8, dashed] plot[variable=\x,  domain=-5:-0.1,samples=50,smooth] (\x,  {ln(cosh(\x))/(\x-tanh(\x))},  1);
     \draw[color=black, line width=0.8, dashed] plot[variable=\x,  domain=0.1:5,samples=50,smooth] (\x,  {ln(cosh(\x))/(\x-tanh(\x))},  1);
     \node (a) at (2.5,-2) {$c=\frac{\log(\cosh(a))}{a-\tanh(a)}$};
     \node (b) at (-1,2) {$a=0$};
     \draw[->] (a) -- (3, {ln(cosh(3))/(3-tanh(3))-0.2});
     \draw[->] (a) -- (-0.25,{ln(cosh(-0.4))/(-0.4-tanh(-0.4))}); 
\end{axis}
\end{tikzpicture}
\end{subfigure}
\caption{Graph of the partial derivatives of $\mathcal{F}\circ\Phi_\text{NN}$ for the analytic case of study \eqref{Chapter1_case_study}. Dashed curves indicate vanishing regions.}
\label{Chapter1_analytic_gradF}
\end{figure}

\pagebreak

The following statements expose a series of properties of this case of study:

\begin{enumerate}
\item The architecture $u_\text{NN}$ posseses \emph{arbitrary precision approximation capacity},  which means that $u^*_\text{NN}=u^*$.
\begin{proof}
Let $c=1$.  Then,  it is straightforward to check that $(\mathcal{F}\circ\Phi_\text{NN})(a,1)$ converges to zero as $a\to \infty$,  which implies that $\Phi_\text{NN}(1,a)$ converges to $u^*$ as $a\to \infty$.
\end{proof}
\item The set of realizations $\mathbb{U}_\text{NN}$ is \emph{non-closed}.
\begin{proof}
The optimal realization $u_\text{NN}^*\in L^2(X)\setminus C^\infty(X)$ is unattainable because $\Phi_\text{NN}(a,c)\in C^\infty(X)$ for all $a,c\in\mathbb{R}$.
\end{proof}
\item The realization map $\Phi_\text{NN}$ is non-injective.  In particular,  the sequence of learnable parameters whose images through $\Phi_\text{NN}$ converge to $u^*_\text{NN}$ is non-unique, although the limit realization $u^*_\text{NN}$ is unique.
\begin{proof}
The odd symmetry of $\tanh(x)$ implies $\Phi_\text{NN}(a,c)=\Phi_\text{NN}(-a,-c)$ for all $(a,c)\in\Theta$,  which shows the non-injectivity.  Then, for $c= 1$, we find distinct sequences $\{(a,1)\}_{a\geq 1}$ and $\{(-a,-1)\}_{a\geq 1}$ of learnable parameters with distinct limits but whose images through $\Phi_\text{NN}$ converge to $u^*_\text{NN}$ as $a\to\infty$. The uniqueness of $u^*_\text{NN}$ follows from item 1.  and the well-posedness of the objective-function minimization. 
\end{proof}
\item The set of realizations $\mathbb{U}_\text{NN}$ is \emph{non-convex}.
\begin{proof}
We need to find $0<\lambda<1$ and $a_1,a_2,c_1,c_2\in\mathbb{R}$ such that $f(x)=\lambda c_1\tanh(a_1 x) + (1-\lambda) c_2\tanh(a_2 x)$ is unrealizable via $\Phi_\text{NN}$, i.e.,  it is not of the form $\Phi_\text{NN}(a,c)=u_\text{NN}(x;a,c) = c\tanh(a x)$ for any $a,c\in\mathbb{R}$.  Indeed,  let $\lambda=1/2$,  $c_1=c_2=2$, $a_1=2$, and $a_2=-1$.  Then,  $f(x)=\tanh(2x)-\tanh(x)$,  which is neither constant nor strict monotonic on $X$.  Because $u_\text{NN}(x;a,c)$ is either strict monotonic or constant on $X$,  $f(x)$ is unrealizable via $\Phi_\text{NN}$.
\end{proof}
\item $\mathcal{F}$ is \emph{convex} on $\mathbb{U}$,  but  $\mathcal{F}\circ\Phi_\text{NN}$ is \emph{non-convex} on $\Theta$.
\begin{proof}
Let $0\leq \lambda\leq 1$ and $u_1,u_2\in\mathbb{U}$. Then,  the triangular inequality $\Vert \lambda(u_1-u^*) + (1-\lambda)(u_2-u^*) \Vert_{L^2(X)}\leq \lambda\Vert u_1-u^*\Vert_{L^2(X)} + (1-\lambda)\Vert u_2-u^*\Vert_{L^2(X)}$ implies $\mathcal{F}(\lambda u_1+(1-\lambda)u_2)\leq \lambda \mathcal{F}(u_1)+(1-\lambda)\mathcal{F}(u_2)$, which shows the convexity of $\mathcal{F}$.  To show the non-convexity of $\mathcal{F}\circ\Phi_\text{NN}$,  fix any $c\neq 0$ and study the curvature of $f_c(a):=(\mathcal{F}\circ\Phi_\text{NN})(a,c)$---recall \Cref{Chapter1_analytic_F}.  For example,  $f''_{1}(a)$ is positive when $a>0$ and negative when $a<-1$.
\end{proof}
\item The negative gradient field posseses undesirable attractive basin regions that lead to poor results when performing the gradient-descent method.
\begin{proof}
The only parameter configurations that lead to desirable realizations occur when $c=\pm 1$ and $a\to\pm\infty$,  which coherently imply $\frac{\partial(\mathcal{F}\circ\Phi_\text{NN})}{\partial\{a,c\}}(a,\pm 1)\to(0,0)$ as $a\to\pm\infty$.  However, we can also obtain near-zero gradients in undesirable parameter configurations. \Cref{Chapter1_analytic_F_flow} shows poor gradient-descent performances that get trapped in near-zero-gradient regions. 
\end{proof}

\begin{figure}[htbp]
\centering
\begin{subfigure}{\textwidth}
\centering
\begin{tikzpicture}
\begin{axis}[width=0.7*\textwidth, view = {45}{55},  colorbar,  colorbar style={fill opacity=0.4, tick label style={opacity=1}}, xlabel={$a$},  ylabel = {$c$}, zlabel={$(\mathcal{F}\circ\Phi_\text{NN})(a,c)$},%
    declare function={f(\x,\y)= 2*(1+\y^2)-(4*\y*ln(cosh(\x))+2*\y^2*tanh(\x))/\x;}]

 \addplot3[surf, opacity=0.4, domain=-5:5,samples=50,%shader=interp
 ]{f(x,y)};
 \edef\myx{-2.5} % first x coordinate
 \edef\myy{4.8} % first y coordinate
 \edef\mystep{-0.05}% negative values mean descending
 \pgfmathsetmacro{\myf}{f(\myx,\myy)}
 \edef\lstCoords{(\myx,\myy,\myf)}
 \pgfplotsforeachungrouped\X in{0,...,200}
 {
 \pgfmathsetmacro{\myx}{\myx+\mystep*xgrad(\myx,\myy)}
 \pgfmathsetmacro{\myy}{\myy+\mystep*ygrad(\myx,\myy)}
 \pgfmathsetmacro{\myf}{f(\myx,\myy)}
 \edef\lstCoords{\lstCoords\space (\myx,\myy,\myf)}
 }
 \addplot3[samples y=0,arrowed, line width=.6, shader=interp] coordinates \lstCoords;
 \edef\myx{-4.5} % first x coordinate
 \edef\myy{4.8} % first y coordinate
 \edef\mystep{-0.1}% negative values mean descending
 \pgfmathsetmacro{\myf}{f(\myx,\myy)}
 \edef\lstCoords{(\myx,\myy,\myf)}
 \pgfplotsforeachungrouped\X in{0,...,200}
 {
 \pgfmathsetmacro{\myx}{\myx+\mystep*xgrad(\myx,\myy)}
 \pgfmathsetmacro{\myy}{\myy+\mystep*ygrad(\myx,\myy)}
 \pgfmathsetmacro{\myf}{f(\myx,\myy)}
 \edef\lstCoords{\lstCoords\space (\myx,\myy,\myf)}
 }
 \addplot3[samples y=0,arrowed, line width=.6, shader=interp] coordinates \lstCoords;
  \edef\myx{3} % first x coordinate
 \edef\myy{4.5} % first y coordinate
 \edef\mystep{-0.1}% negative values mean descending
 \pgfmathsetmacro{\myf}{f(\myx,\myy)}
 \edef\lstCoords{(\myx,\myy,\myf)}
 \pgfplotsforeachungrouped\X in{0,...,200}
 {
 \pgfmathsetmacro{\myx}{\myx+\mystep*xgrad(\myx,\myy)}
 \pgfmathsetmacro{\myy}{\myy+\mystep*ygrad(\myx,\myy)}
 \pgfmathsetmacro{\myf}{f(\myx,\myy)}
 \edef\lstCoords{\lstCoords\space (\myx,\myy,\myf)}
 }
 \addplot3[samples y=0,arrowed, line width=.6, shader=interp] coordinates \lstCoords;
% \edef\myx{2.5} % first x coordinate
% \edef\myy{-4.8} % first y coordinate
% \edef\mystep{-0.03}% negative values mean descending
% \pgfmathsetmacro{\myf}{f(\myx,\myy)}
% \edef\lstCoords{(\myx,\myy,\myf)}
% \pgfplotsforeachungrouped\X in{0,...,100}
% {
% \pgfmathsetmacro{\myx}{\myx+\mystep*xgrad(\myx,\myy)}
% \pgfmathsetmacro{\myy}{\myy+\mystep*ygrad(\myx,\myy)}
% \pgfmathsetmacro{\myf}{f(\myx,\myy)}
% \edef\lstCoords{\lstCoords\space (\myx,\myy,\myf)}
% }
% \addplot3[samples y=0,arrowed, line width=.6, shader=interp] coordinates \lstCoords;
%  \edef\myx{4} % first x coordinate
% \edef\myy{-4.8} % first y coordinate
% \edef\mystep{-0.1}% negative values mean descending
% \pgfmathsetmacro{\myf}{f(\myx,\myy)}
% \edef\lstCoords{(\myx,\myy,\myf)}
% \pgfplotsforeachungrouped\X in{0,...,100}
% {
% \pgfmathsetmacro{\myx}{\myx+\mystep*xgrad(\myx,\myy)}
% \pgfmathsetmacro{\myy}{\myy+\mystep*ygrad(\myx,\myy)}
% \pgfmathsetmacro{\myf}{f(\myx,\myy)}
% \edef\lstCoords{\lstCoords\space (\myx,\myy,\myf)}
% }
% \addplot3[samples y=0,arrowed, line width=.6, shader=interp] coordinates \lstCoords;
\end{axis}
\end{tikzpicture}
\end{subfigure}
\vskip 2em
\begin{subfigure}{\textwidth}
\centering
\begin{tikzpicture}
\begin{axis}[width=0.7*\textwidth, view = {0}{90},  xmin=-5,xmax=5,ymin=-5,ymax=5, colorbar,  colorbar style={fill opacity=0.5,  tick label style={opacity=1}},  xlabel={$a$},  ylabel = {$c$}, zlabel={$(\mathcal{F}\circ\Phi_\text{NN})(a,c)$},title={$(\mathcal{F}\circ\Phi_\text{NN})(a,c)$},%
declare function={f(\x,\y)= 2*(1+\y^2)-(4*\y*ln(cosh(\x))+2*\y^2*tanh(\x))/\x;}]

\draw[color=red, line width=1, dashed] plot[variable=\x,  domain=-5:-0.1,samples=50,smooth] (\x,  {ln(cosh(\x))/(\x-tanh(\x))},  1);
\draw[color=red, line width=1, dashed] plot[variable=\x,  domain=0.1:5,samples=50,smooth] (\x,  {ln(cosh(\x))/(\x-tanh(\x))},  1);
\draw[color=red, line width=1, dashed] plot[variable=\x,  domain=-5:5,samples=50,smooth] (0,\x, 1);
\draw[color=blue, line width=1, dashed] plot[variable=\x,  domain=-5:-0.1,samples=50,smooth] (\x,  {2*( ln(cosh(\x)) - \x * tanh(\x) ) / ( \x * ( 1 - (tanh(\x))^2 ) - tanh(\x) )},  1);
\draw[color=blue, line width=1, dashed] plot[variable=\x,  domain=0.1:5,samples=50,smooth] (\x,  {2*( ln(cosh(\x)) - \x * tanh(\x) ) / ( \x * ( 1 - (tanh(\x))^2 ) - tanh(\x) )},  1);
\draw[color=blue, line width=1, dashed] plot[variable=\x,  domain=-5:5,samples=50,smooth] (\x, 0, 1);

 \addplot3[surf, opacity=0.4, domain=-5:5,samples=50,shader=interp
 ]{f(x,y)};
 \edef\myx{-2.5} % first x coordinate
 \edef\myy{4.8} % first y coordinate
 \edef\mystep{-0.05}% negative values mean descending
 \pgfmathsetmacro{\myf}{f(\myx,\myy)}
 \edef\lstCoords{(\myx,\myy,\myf)}
 \pgfplotsforeachungrouped\X in{0,...,200}
 {
 \pgfmathsetmacro{\myx}{\myx+\mystep*xgrad(\myx,\myy)}
 \pgfmathsetmacro{\myy}{\myy+\mystep*ygrad(\myx,\myy)}
 \pgfmathsetmacro{\myf}{f(\myx,\myy)}
 \edef\lstCoords{\lstCoords\space (\myx,\myy,\myf)}
 }
 \addplot3[samples y=0,arrowed, line width=.6, shader=interp] coordinates \lstCoords;
 \edef\myx{-4.5} % first x coordinate
 \edef\myy{4.8} % first y coordinate
 \edef\mystep{-0.1}% negative values mean descending
 \pgfmathsetmacro{\myf}{f(\myx,\myy)}
 \edef\lstCoords{(\myx,\myy,\myf)}
 \pgfplotsforeachungrouped\X in{0,...,200}
 {
 \pgfmathsetmacro{\myx}{\myx+\mystep*xgrad(\myx,\myy)}
 \pgfmathsetmacro{\myy}{\myy+\mystep*ygrad(\myx,\myy)}
 \pgfmathsetmacro{\myf}{f(\myx,\myy)}
 \edef\lstCoords{\lstCoords\space (\myx,\myy,\myf)}
 }
 \addplot3[samples y=0,arrowed, line width=.6, shader=interp] coordinates \lstCoords;
  \edef\myx{3} % first x coordinate
 \edef\myy{4.5} % first y coordinate
 \edef\mystep{-0.1}% negative values mean descending
 \pgfmathsetmacro{\myf}{f(\myx,\myy)}
 \edef\lstCoords{(\myx,\myy,\myf)}
 \pgfplotsforeachungrouped\X in{0,...,100}
 {
 \pgfmathsetmacro{\myx}{\myx+\mystep*xgrad(\myx,\myy)}
 \pgfmathsetmacro{\myy}{\myy+\mystep*ygrad(\myx,\myy)}
 \pgfmathsetmacro{\myf}{f(\myx,\myy)}
 \edef\lstCoords{\lstCoords\space (\myx,\myy,\myf)}
 }
 \addplot3[samples y=0,arrowed, line width=.6, shader=interp] coordinates \lstCoords;
 \edef\myx{2.5} % first x coordinate
 \edef\myy{-4.8} % first y coordinate
 \edef\mystep{-0.03}% negative values mean descending
 \pgfmathsetmacro{\myf}{f(\myx,\myy)}
 \edef\lstCoords{(\myx,\myy,\myf)}
 \pgfplotsforeachungrouped\X in{0,...,200}
 {
 \pgfmathsetmacro{\myx}{\myx+\mystep*xgrad(\myx,\myy)}
 \pgfmathsetmacro{\myy}{\myy+\mystep*ygrad(\myx,\myy)}
 \pgfmathsetmacro{\myf}{f(\myx,\myy)}
 \edef\lstCoords{\lstCoords\space (\myx,\myy,\myf)}
 }
 \addplot3[samples y=0,arrowed, line width=.6, shader=interp] coordinates \lstCoords;
  \edef\myx{4} % first x coordinate
 \edef\myy{-4.8} % first y coordinate
 \edef\mystep{-0.1}% negative values mean descending
 \pgfmathsetmacro{\myf}{f(\myx,\myy)}
 \edef\lstCoords{(\myx,\myy,\myf)}
 \pgfplotsforeachungrouped\X in{0,...,200}
 {
 \pgfmathsetmacro{\myx}{\myx+\mystep*xgrad(\myx,\myy)}
 \pgfmathsetmacro{\myy}{\myy+\mystep*ygrad(\myx,\myy)}
 \pgfmathsetmacro{\myf}{f(\myx,\myy)}
 \edef\lstCoords{\lstCoords\space (\myx,\myy,\myf)}
 }
 \addplot3[samples y=0,arrowed, line width=.6, shader=interp] coordinates \lstCoords;
\end{axis}
\end{tikzpicture}
\end{subfigure}
\vskip 1em
\begin{subfigure}{\textwidth}
\centering
\begin{tikzpicture}
\begin{axis}[hide axis,
	    xmin=-0.1,
	    xmax=1.1,
	    ymin=-0.1,
	    ymax=1.1,
	 	legend style={anchor=north, /tikz/every even column/.append style={row sep=0.25cm}},
	 	legend columns = 1
            ]

    	\addlegendimage{color=blue, line width=1, dashed};
	\addlegendentry{$\left\lbrace(a,c)\in\Theta:\frac{\partial(\mathcal{F}\circ\Phi_\text{NN})}{\partial a}(a,c)=0\right\rbrace$};
	\addlegendimage{color=red, line width=1, dashed};
	\addlegendentry{$\left\lbrace(a,c)\in\Theta:\frac{\partial(\mathcal{F}\circ\Phi_\text{NN})}{\partial c}(a,c)=0\right\rbrace$};
    \addlegendimage{color=white, line width=1, dashed};
\end{axis}
\end{tikzpicture}
\end{subfigure}
\caption{Different performances of the gradient-descent method for the analytic case of study \eqref{Chapter1_case_study}. We maintain constant the learning rates in all cases and carry out $200$ gradient-descent iterations.}
\label{Chapter1_analytic_F_flow}
\end{figure}
\end{enumerate}

At the discretization level,  we approximate $\mathcal{F}\circ\Phi_\text{NN}$ via a loss function  that we expect to inherit similar conditions than above.  Indeed, let $\mathbf{x}=\{x_i\}_{i=1}^N\subset X$. Then, 
\begin{subequations}
\begin{align}
(\mathcal{F}\circ\Phi_\text{NN})(a,c)\approx \mathcal{L}(a,c;\mathbf{x}) &= \sum_{i=1}^N \omega_i (c\tanh(ax_i)\pm 1)^2,\\
\frac{\partial(\mathcal{F}\circ\Phi_\text{NN})}{\partial a}(a,c)\approx \frac{\partial \mathcal{L}}{\partial a}(a,c;\mathbf{x}) &= 2ac \sum_{i=1}^N \omega_i  (c\tanh(a x_i)\pm 1)\;\text{sech}^2(a x_i),\\
\frac{\partial(\mathcal{F}\circ\Phi_\text{NN})}{\partial c}(a,c)\approx \frac{\partial \mathcal{L}}{\partial c}(a,c;\mathbf{x}) &= 2 \sum_{i=1}^N \omega_i (c\tanh(a x_i)\pm 1) \tanh(a x_i),
\end{align}
\end{subequations} where $\omega_i$ denotes the integration weight related to the integration point $x_i$, and where the positive or negative sign depends on whether $x_i$ is negative or positive, respectively.

When $c=\pm 1$ and $a\to \pm\infty$, we obtain the desired realizations convergence $\Phi_\text{NN}(a,c)\to u^*$ with coherent
\begin{equation}
\frac{\partial \mathcal{L} }{\partial\{a,c\}}(a,\pm 1;\mathbf{x}) \to (0,0) \text{ as } a\to\pm\infty, \quad \text{for any } \mathbf{x}\in X^N  \text{ and } N>0.
\end{equation} However,  $\frac{\partial \mathcal{L} }{\partial\{a,c\}}(0,c;\mathbf{x})=(0,0)$ for any $c\in\mathbb{R},  \mathbf{x}\in X^N  \text{ and } N>0$,  but $\Phi_\text{NN}(0,c) = 0\neq u^*$ for all $c\in\mathbb{R}$.  Hence,  parameters of the form $(0,c)\in\Theta$ are undesirable critical points susceptible to trap the learnable parameters during a stochastic gradient-descent training.
